Optimal Flexible Consensus and its Application to Ethereum

Classic BFT consensus protocols guarantee safety and liveness for all clients if fewer than one-third of replicas are faulty. However, in applications such as high-value payments, some clients may want to prioritize safety over liveness. Flexible consensus allows each client to opt for a higher safety resilience, albeit at the expense of reduced liveness resilience. We present the first construction that allows optimal safety--liveness tradeoff for every client simultaneously. This construction is modular and is realized as an add-on applied on top of an existing consensus protocol. The add-on consists of an additional round of voting and permanent locking done by the replicas, to sidestep a sub-optimal quorum-intersection-based constraint present in previous solutions. We adapt our construction to the existing Ethereum protocol to derive optimal flexible confirmation rules that clients can adopt unilaterally without requiring system-wide changes. This is possible because existing Ethereum protocol features can double as the extra voting and locking. We demonstrate an implementation using Ethereum's consensus API.

==> figures/protocol-views-_utils.tex <==
\tikzset{fig_protocol_views/.style={
            x=0.9cm,
            y=0.5cm,
            node distance=0.5cm,
            %
            block/.style = {
                    minimum width=0.5cm,
                    minimum height=0.5cm,
                    draw,
                    shade,
                    top color=white,
                    bottom color=black!10,
                    inner sep=0,
                },
            block-adv/.style = {
                    block,
                    bottom color=myParula07Red!50,
                    draw=myParula07Red!50!black,
                },
            block-hon/.style = {
                    block,
                    bottom color=myParula05Green!50,
                    draw=myParula05Green!50!black,
                },
            link/.style = {
                    -latex,
                },
            link-adv/.style = {
                    link,
                },
            link-hon/.style = {
                    link,
                },
            vote/.style = {
                    pos11/.style = { xshift=-0.25cm, yshift=+0.30cm, },
                    pos12/.style = { xshift= 0.00cm, yshift=+0.30cm, },
                    pos13/.style = { xshift=+0.25cm, yshift=+0.30cm, },
                    pos21/.style = { xshift=-0.25cm, yshift=+0.00cm, },
                    pos22/.style = { xshift= 0.00cm, yshift=+0.00cm, },
                    pos23/.style = { xshift=+0.25cm, yshift=+0.00cm, },
                    pos31/.style = { xshift=-0.25cm, yshift=-0.30cm, },
                    pos32/.style = { xshift= 0.00cm, yshift=-0.30cm, },
                    pos33/.style = { xshift=+0.25cm, yshift=-0.30cm, },
                },
            votelabel/.style = {
                    align=center,
                    above/.style = {
                            yshift=+0.7cm,
                        },
                    below/.style = {
                            yshift=-0.7cm,
                        },
                },
            locked/.style = {
                    xshift=0.25cm,
                    yshift=-0.25cm,
                },
        }}

==> lib/_spacinghacks.tex <==
%
%
%
%

%
%
%
%

%
%
%
%

%
%

%
%
%
%
%
%
%
%
%
%
%

%
%
%

%
%
%
%
%








%
%
%
%

%
%

%
%
%
%

%
%
%

%
%
%
%
%


